ShadowNav: Crater-Based Localization for Nighttime and Permanently Shadowed Region Lunar Navigation

There has been an increase in interest in missions that drive significantly longer distances per day than what has currently been performed. Further, some of these proposed missions require autonomous driving and absolute localization in darkness. For example, the Endurance A mission proposes to drive 1200km of its total traverse at night. The lack of natural light available during such missions limits what can be used as visual landmarks and the range at which landmarks can be observed. In order for planetary rovers to traverse long ranges, onboard absolute localization is critical to the ability of the rover to maintain its planned trajectory and avoid known hazardous regions. Currently, to accomplish absolute localization, a ground in the loop (GITL) operation is performed wherein a human operator matches local maps or images from onboard with orbital images and maps. This GITL operation limits the distance that can be driven in a day to a few hundred meters, which is the distance that the rover can maintain acceptable localization error via relative methods. Previous work has shown that using craters as landmarks is a promising approach for performing absolute localization on the moon during the day. In this work we present a method of absolute localization that utilizes craters as landmarks and matches detected crater edges on the surface with known craters in orbital maps. We focus on a localization method based on a perception system which has an external illuminator and a stereo camera. We evaluate (1) both monocular and stereo based surface crater edge detection techniques, (2) methods of scoring the crater edge matches for optimal localization, and (3) localization performance on simulated Lunar surface imagery at night. We demonstrate that this technique shows promise for maintaining absolute localization error of less than 10m required for most planetary rover missions.

==> reviews.tex <==
{
\color{blue}
\textbf{Reviews}
\begin{enumerate}
    \item This is a great paper with good technical content and a sufficient amount of experiments. The purpose of this paper is very challenging which is shown in the experimental results. Look forward to the extended work in the future. 
    \item Great job on this paper, it is well-written and organized with technical content. Recommend making figures 9, 10 and 11 larger for enhanced readability. Try using full width across both columns to enable reading of the text. IEEE format also required that the descriptive text for figures and tables to be bolded. Great job!
    \item Use bolded text for the figure descriptions. Same as you did for the tables.
    \item Excellent work evaluating the use of different detectors with rover-like imagery; I think your paper would benefit from a more thorough description of your "crater matching" process. You deeply describe your detection process, but I only found 1-2 sentences on matching to known craters, and the *global* part of this localization problem is what's so important. Perhaps adding a small results section detailing how well your particle filter performed matching to "known craters" would solve that issue. It you don't have that metric or similar, call that out as future work.
\end{enumerate}
}
